Multi-Task Combinatorial Bandits for Budget Allocation

Today's top advertisers typically manage hundreds of campaigns simultaneously and consistently launch new ones throughout the year. A crucial challenge for marketing managers is determining the optimal allocation of limited budgets across various ad lines in each campaign to maximize cumulative returns, especially given the huge uncertainty in return outcomes. In this paper, we propose to formulate budget allocation as a multi-task combinatorial bandit problem and introduce a novel online budget allocation system. The proposed system: i) integrates a Bayesian hierarchical model to intelligently utilize the metadata of campaigns and ad lines and budget size, ensuring efficient information sharing; ii) provides the flexibility to incorporate diverse modeling techniques such as Linear Regression, Gaussian Processes, and Neural Networks, catering to diverse environmental complexities; and iii) employs the Thompson sampling (TS) technique to strike a balance between exploration and exploitation. Through offline evaluation and online experiments, our system demonstrates robustness and adaptability, effectively maximizing the overall cumulative returns. A Python implementation of the proposed procedure is available at https://anonymous.4open.science/r/MCMAB.

==> 1.Introduction.tex <==
\section{Introduction}
Today’s top advertisers can run hundreds of simultaneous campaigns with overlapping goals, and this creates a challenge for the teams that manage performance before and during a campaign. In a major Demand Side Platform (DSP) like Amazon DSP these campaigns each have various tactics called ad-lines which specify target audiences to reach, publishers, devices, creatives, campaign shares of budget, and other delivery settings. An advertiser may manage thousands of ad lines across all campaigns. One such advertiser is Amazon with a group that manages marketing activities of more than a hundred different marketing teams that often have similar goals such as to drive traffic to its retail site or to drive product purchases. These advertisers invest a significant amount or their marketing budget on a single DSP and for that reason they have the opportunity to drive more value by optimizing the signals they have on this stream of data.

One of the opportunities they have is to coordinate the activities of multiple in-flight campaigns which have similar objectives. For instance, the advertiser may run multiple campaigns simultaneously to drive retail website traffic with different creative messaging. They depend on automated performance management tools to support these activities. DSPs employ automated in-flight performance optimizations that respond to signals on its own spend and conversion data within a single campaign. These DSPs are not designed to coordinate signals across the multitude of campaigns each advertiser runs in real-time. Advertisers have spend and conversion signals coming in from multiple campaigns all the time. Today, this cross-campaign coordination falls on individual advertisers to take action on.  Data-driven advertisers are inundated with data streaming into dashboards and will use reactive performance optimization tools to respond to this. Even the best of them may miss opportunities to tune each campaign in response to the data from others. We were motivated by the challenge to address this opportunity, so we can provide a performance improving solution to advertisers who manage multiple campaigns at the same time. 

A second opportunity is to apply learnings from past campaigns to future campaigns. When a new campaign is started, the ad-lines in a campaign start off with each with a percent of the campaign budget based on predictions before the campaign starts. While campaigns are in-flight, automated tools can dynamically reallocate budgets, but it can take as much as 3 weeks to find the right budget allocation mix. While the DSP provides some tools to help marketing managers set a budget allocation, they lack the ability to rapidly evolve the recommended mix for subsequent campaigns based on previous ones. This is a second motivation for us to investigate this method of cross-campaign learning. 

In addition to solving the problem, we were motivated to find a solution that can address the reality that the advertising environment changes rapidly.  We should consider that i) many of the current optimization methods rely solely on historical data, failing to address the uncertainty of changing environments (i.e., users' preferences, etc.) and ii) potential heterogeneity among adlines/campaigns may exist, which means that even two ad-lines with identical features may perform differently. The DSP facilitates auctions among many different supply sources so that advertisers can bid for inventory across a variety of publishers in real-time. Some of the changes that we want to account for are changes due to seasonality, available ad supply, competitive bidding behavior, privacy regulations, DSP functionality, and customer behaviors. Advertisers reported that it is common to intervene with campaigns in-flight as well, which is a mechanism to respond to changes in the advertising and business environments. An algorithm that can respond and adapt quickly to change will solve a pain point that advertisers have in algorithms that depend too heavily on past performance. 



(To edit) In the real-world advertising market, major Demand Side Platforms (DSPs) like Amazon DSP typically manage tens of thousands of ads campaigns requested by various advertisers. Meanwhile, these platforms also maintain a large and diverse portfolio of ad lines, allowing advertisers to compose their campaigns selectively. With budget limit specified by the advertiser of each ads campaign, the ultimate objective remains consistent across all campaigns: to optimize the allocation of this limited budget among the selected ad lines in order to maximize returns, such as Return on Investment (ROI). This problem is widely studied as a pure optimization problem \citep{karlsson2020feedback, geng2021automated}[more references to be added]. However, two significant limitations are frequently observed in the systems deployed within existing DSPs: (1) Relying solely on past performance to predict future outcomes frequently results in unreliable estimations, particularly when faced with a high degree of statistical uncertainty in the measurement of outcomes and rapidly evolving context; and (2) Treating each ad campaign as an isolated task and learning optimal budget allocation strategies from scratch for each one not only lacks the capability of providing informative budget initialization, but also requires considerable time to develop effective budget allocation strategies, especially when a large set of ad lines is under consideration.


Recent literature has attempted to address these limitations. For example, \citet{nuara2018combinatorial} and \citet{zuo2021combinatorial} formulated the budget/resource allocation problem as a combinatorial multi-armed bandit problem, intelligently balancing exploration and exploitation to account for the uncertainty in the reward distributions of each ad line. \citet{han2020contextual} introduced a contextual bandit framework that further shares information across ad lines, but based on a strong model assumption. However, it is worth noting that the approaches in the aforementioned studies are all formulated from the \textit{advertiser's perspective}, while our focus is on the \textit{DSP's perspective}. Adopting to the perspective of DSPs as central platforms allows us to learn the reward distribution of each (campaign, ad line) tuple more efficiently by leveraging the detailed information on a diverse range of ads campaigns from various advertisers. Although informative data are available to be utilized, how to efficiently share information among the large number ads campaigns is known to be challenging.

We present a meta-bandit framework to address both identified limitations simultaneously. Specifically, on the basis of the combinatorial MAB framework introduced in \citet{nuara2018combinatorial} and \citet{zuo2021combinatorial}, we propose to formulate the budget optimization problem as a multi-task combinatorial MAB, where each ads campaign is a single task, and each task is a combinatorial MAB. In general, there are three major steps involved: (1) \textbf{Intelligent Information Sharing}: We employ a feature-based Bayesian hierarchical model to estimate the reward distributions, sharing information across both ads campaigns and ad lines while accounting for the inter-campaign and inter-ad-line heterogeneity, (2) \textbf{Efficient Exploration}: Using Thompson Sampling, the system is enabled to gather diverse data, thereby enhancing the accuracy of the reward distribution estimates and, consequently, the performance of budget allocation, and (3) \textbf{Optimization}: The actual allocation of budgets based on the estimated rewards obtained in previous steps. 


\textbf{Motivation}
\begin{enumerate}
    \item \textbf{Business}
    \begin{enumerate}
        \item fail to allow exploration: solely relying on past performance is frequently unreliable, easily resulted in suboptimal recommendation (necessity of striking a good balance between exploration and exploitation)
        
        \item lack of information sharing in the existing framework: inefficient budget initialization and inefficient learning (most campaigns last 1-2 months with limited observations)
        
        \item fail to address the potential heterogeneity: it exists, performance from similar adlines may not be representative
    \end{enumerate}
    \item \textbf{Methodology (comparing the lit related to the ADs budget allocation)}
    \begin{enumerate}
        \item combinatorial bandits in budget allocation: exisitng work fail to do information sharing among different campaign/adlines--inefficient 
        \item contextual bandits in budget allocation: the paper employs a strong log-linear model assumption, and assume that the global model is reliable (It is an implicit assumption. They update the local model based on an augmented dataset consisting of past observations and data points generated by the global model. Given the scarcity of historical data, the generated data would dominate the posterior distribution of the local model.)---> the posterior updating process is time cost in practice, as it will keep sampling the parameters until the sampled parameters meet the criteria
        \item meta bandits: never being used in the specific application, never incorporating with advanced non-parametric regression models
    \end{enumerate}
\end{enumerate}

==> 1.Introduction_new.tex <==
\section{Introduction}

Budget allocation has been given wide attention in various fields across advertising market, clinical trial, transportation, and more. It is always interested for decision makers to learn an optimal strategy that can optimize the overall reward given limited resources such as cash flow, time and population. For example, in advertising market, major Demand Side Platforms (DSP) like Amazon DSP routinely manage multiple concurrent campaigns, each comprising various tactics—such as ad-lines—which delineate target audiences, publishers, devices, creatives, campaign budget shares, and other delivery settings. Given specified amount of budget at each day, the decision maker will learn from the past data and decides the allocation strategy across campaigns and the corresponding ad lines.

The traditional literature often address this problem from a purist optimization’s perspective, as exemplified by works like \citet{karlsson2020feedback, geng2021automated}. For example, \citet{karlsson2020feedback} formalize budgets as a hard constraint to optimize specified campaign objectives, such as conversions or revenue. Although intuitively feasible, this type of approach often results in suboptimal solutions in a sequential decision making problem due to its pure reliance on historical data. Therefore, how to strike a good balance between exploration and exploitation becomes a critical problem to deal with.

 As a powerful tool for online decision-making, bandit algorithms offer an elegant solution to the exploration-exploitation tradeoff. To address the inherent resource constraints in budget allocation problems, a novel line of work has formalized the budget allocation problem from combinatorial bandits' perspective \citep{zuo2021combinatorial, nuara2018combinatorial, nuara2022online}. This framework discretizes budgets into finite proportions, aligning with the inherent nature of combinatorial bandits in slate recommendation. Notably, in contrast to treating the budget as a continuous variable, real-world allocation naturally involves dividing the budget into proportions prior to allocation. More importantly, this approach eliminates the need for imposing any smoothness assumptions when discretizing the budget, which will be detailed in the following section.
 
 
 Although it is conceptually feasible to borrow the combinatorial bandits framework in budget allocation, existing methodologies prove too idealistic to handle the following two challenges that are often encountered in real scenarios:

%There are two representative challenges that failed to be addressed in existing work:

\textbf{Challenge 1: Information sharing across large campaigns} 
Today’s top advertisers can manage hundreds of simultaneous campaigns with overlapping goals, which creates a substantial challenge for demand side platforms to optimize performance before and during a campaign. This situation can be further divided into two cases: 1) multiple campaigns going concurrently at the same round, or 2) campaigns coming sequentially one after the other. Nowadays, budget allocation usually occurs independently at the campaign level, with specific budget proportions attributed sequentially to each ad line within campaigns. While it's straightforward for models to consider budget allocation directly from the ad line level, this approach may overlook valuable shared information between different campaigns. For instance, ad lines across various campaigns may have similar contextual information or goals, such as attribution channels or objectives like driving traffic to a retail site or boosting product purchases. Therefore, how to efficiently leverage this shared information to enhance the learning of a more effective budget allocation policy remains an ongoing inquiry.

%[need to be incorporated together with the last paragraph]
%A second opportunity is to apply learnings from past campaigns to future campaigns. When a new campaign is started, the ad-lines in a campaign start off with each with a percent of the campaign budget based on predictions before the campaign starts. While campaigns are in-flight, automated tools can dynamically reallocate budgets but it can take as much as 3 weeks to find the right budget allocation mix. While the DSP provides some tools to help Marketing Managers setup a budget allocation, they lack the ability to rapidly evolve the recommended mix for subsequent campaigns based on past ones. This is a second motivation for us to research this method of cross campaign learning. 


\textbf{Challenge 2: Addressing heterogeneity between ad lines} 
In reality where the advertising environment is evolving rapidly, the performances of two ad lines can vary significantly even when they share identical features. Some of the changes that we want to account for are changes to seasonality, available ad supply, competitive bidding behavior, privacy regulations, DSP functionality, and customer behaviors. As is shown in Figure \ref{fig:intro_3}, the distribution of clicks (reward) varies among different ad lines even when all of the contextual information are fixed and identical. Advertisers reported that it is common to intervene with campaigns in-flight as well, which is a mechanism to respond to changes in the advertising and business environments. Therefore, it is important to develop an algorithm that is capable of responding and adapting quickly to such changes and accounting for potential heterogeneity that cannot be measured through observed contextual information.



In the past few years, there has been some literature trying to address the above two challenges. For example, %\citet{nuara2018combinatorial} and \citet{zuo2021combinatorial} formulated the budget/resource allocation problem as a combinatorial multi-armed bandit problem, intelligently balancing exploration and exploitation to account for the uncertainty in the reward distributions of each ad line. 
\citet{han2020contextual} introduced a contextual bandit framework that is able to share information across ad lines. However, their framework highly relies on a power law form (i.e. log-linearity) assumption, which can be easily violated in a lot of real scenarios. Moreover, the efficacy of their methodology is closely related to how well the global model fits the data, which creates a potential challenge when dealing with limited sample sizes or substantial noise in the data. [to be revised] GP combinatorial bandits


In this paper, we propose a meta-bandit framework based under the framework of combinatorial bandits to address both challenges simultaneously. We formulate the budget optimization problem as a multi-task combinatorial MAB, where each ads campaign represents a single task, and each task is a combinatorial MAB with multiple ad lines and discretized budget proportions to choose. We developed a novel feature-based Bayesian hierarchical model to estimate the reward distributions, sharing information across both ads campaigns and ad lines while accounting for the inter-campaign and inter-ad-line heterogeneity. To handle bandits update, we incorporate our structure with Thompson Sampling (TS) to realize the exploration-exploitation tradeoff. 	The innovations of our methodology is four-fold:

\textbf{First}, we are the very first work to address the multi-task (inter-campaign) budget allocation problem in bandits setup. \textbf{Second}, we utilized a novel Bayesian hierarchical model to handle both across-campaign info sharing and inner-campaign heterogeneity at the same time. \textbf{Third}, our framework allows very flexible reward modeling, including 1) linear mixed effect model, 2) Gaussian process bayesian regression model, and 3) neural network-based Thompson sampling, which released the modeling assumptions such as log-linearity that is often assumed in existing literature.  \textbf{Finally}, we illustrate the performance of our framework from both simulation and real data from Amazon ADA side. All results present that our framework can realize faster convergence, lower regret, and better budget allocation strategy in the long run.

\begin{comment}
\vspace{0.2in}
\textbf{Motivation}
\begin{enumerate}
    \item \textbf{Business}
    \begin{enumerate}
        \item fail to allow exploration: solely relying on past performance is frequently unreliable, easily resulted in suboptimal recommendation (necessity of striking a good balance between exploration and exploitation)
        
        \item lack of information sharing in the existing framework: inefficient budget initialization and inefficient learning (most campaigns last 1-2 months with limited observations)
        
        \item fail to address the potential heterogeneity: it exists, performance from similar adlines may not be representative
    \end{enumerate}
    \item \textbf{Methodology (comparing the lit related to the ADs budget allocation)}
    \begin{enumerate}
        \item combinatorial bandits in budget allocation: exisitng work fail to do information sharing among different campaign/adlines--inefficient 
        \item contextual bandits in budget allocation: the paper employs a strong log-linear model assumption, and assume that the global model is reliable (It is an implicit assumption. They update the local model based on an augmented dataset consisting of past observations and data points generated by the global model. Given the scarcity of historical data, the generated data would dominate the posterior distribution of the local model.)---> the posterior updating process is time cost in practice, as it will keep sampling the parameters until the sampled parameters meet the criteria
        \item meta bandits: never being used in the specific application, never incorporating with advanced non-parametric regression models
    \end{enumerate}
\end{enumerate}
\end{comment}
\begin{figure}[tbh]
  \centering
  \includegraphics[width=\linewidth]{Figs/motiv1.png}
\end{figure}
\begin{figure}[tbh]
  \centering
  \includegraphics[width=\linewidth]{Figs/motiv2.png}
\end{figure}

\begin{figure}[tbh]
  \centering  \includegraphics[width=\linewidth]{Figs/motiv3.png}
  \caption{The distribution of reward (click) for ad lines with the same contextual information}\label{fig:intro_3}
\end{figure}

\begin{comment}
\textbf{Why Discretization?}
business perspective: the campaign manager would prefer to assign by percentages

optimization of the budget allocation problem is complex, while others deal with it by imposing a strong model assumption, we tend to deal with is by discretizing the budget space 
\end{comment}



+ sequential case [YX: I only added one sentence in challenge 1 to explain concurrent setting and sequential setting; feel free to modify anything you think is inappropriate]

+ challenge 1 is the difficulty of reward distribution learning, [YX: may need Lin's help :)]

+ figures to each of the challenge [YX: done for challenge 2]

+ cite another combinatorial bandits paper, which lacks the utilization of the metadata information. [YX: may need Lin's help :)]


[move to the related work] In the past few years, there has been some literature trying to address the above two challenges. For example, \citet{han2020contextual} introduced a contextual bandit framework that is able to share information across ad lines. However, their framework highly relies on a power law form (i.e. log-linearity) assumption, which can be easily violated in a lot of real scenarios. Moreover, the efficacy of their methodology is closely related to how well the global model fits the data, which creates a potential challenge when dealing with limited sample sizes or substantial noise in the data. [to be revised] GP combinatorial bandits

%\citet{nuara2018combinatorial} and \citet{zuo2021combinatorial} formulated the budget/resource allocation problem as a combinatorial multi-armed bandit problem, intelligently balancing exploration and exploitation to account for the uncertainty in the reward distributions of each ad line. 

==> Algorithm/algo_efficient.tex <==
\begin{algorithm}[!t]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{Specification of $g$ and the corresponding prior; known parameters (i.e., $\sigma_\epsilon$, $\Cov$) of the hierarchical model
}
Set $\mH = \{\}$

\For{every decision point t}{ 
Update the posterior for $g$ as $\prob(g|\mH)$, according to the  hierarchical model \eqref{eqn:hierachical_model}\;

Sample a $\tilde{g} \sim \prob(g|\mH)$\;

\For{every campaign m}{
Given $\tilde{g}$, update the posterior for $\vthe_m$ as $\prob(\vthe_m|\tilde{g}, \mH)$\;

Sample an utility vector $\tilde{\vthe}_{m} \sim \prob(\vthe_m|\tilde{g}, \mH)$\; 

Take action $\boldsymbol{a}_{m,t} = argmax_{\boldsymbol{a}_{m,\cdot}\in\mathcal{S}_m} \sum_{k\in [K_m]}\tilde{\theta}_{m,k,a_{m,k,\cdot}}$\;

Receive reward $R_{m,t}$\;

Update the dataset as $\mH \leftarrow \mH \cup \{(m, \boldsymbol{a}_{m,t}, R_{m,t})\}$
}
}
\caption{Computational Efficient MCMAB-Concurrent}\label{alg:TS-concurrent}
\end{algorithm}



\begin{algorithm}[h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{Specification of $g$ and the corresponding prior; known parameters (i.e., $\sigma_\epsilon$, $\Cov$) of the hierarchical model
}
Set $\mH = \{\}$

\For{every campaign m}{ 
Update the posterior for $g$ as $\prob(g|\mH)$, according to the  hierarchical model \eqref{eqn:hierachical_model}\;

Sample a $\tilde{g} \sim \prob(g|\mH)$\;

\For{every decision time t}{

Given $\tilde{g}$, update the posterior for $\vthe_m$ as $\prob(\vthe_m|\tilde{g}, \mH)$\;

Sample an utility vector $\tilde{\vthe}_{m} \sim \prob(\vthe_m|\tilde{g}, \mH)$\; 

Take action $\boldsymbol{a}_{m,t} = argmax_{\boldsymbol{a}_{m,\cdot}\in\mathcal{S}_m} \sum_{k\in [K_m]}\tilde{\theta}_{m,k,a_{m,k,\cdot}}$\;

Receive reward $R_{m,t}$\;

Update the dataset as $\mH \leftarrow \mH \cup \{(m, \boldsymbol{a}_{m,t}, R_{m,t})\}$
}
}
\caption{Computational Efficient MCMAB-Sequential}\label{alg:TS-sequential}
\end{algorithm}

==> info_recycles.tex <==
Unfortunately, this problem still remains unsolved in the literature due to the following complexities:

1. Since budget itself is continuous (or at least has a large number of arms even after discretization), how to develop a scalable bandits algorithm that can balance exploration-exploitation tradeoff and find the optimal policy would be very challenging.
2. Unlike the traditional MAB or CB problems, the resource constraint is always present in each ads campaign, and should be satisfied at each round of bandits update.
3. Although the naive way is to regard each campaign as a separate bandits problem so that multiple campaigns can be updated at the same time, how to develop an integrated multi-task bandits algorithm that allows for information sharing between each single task is still an open question in the context of budget allocation.


Let am,t​=(am,1,t​,⋯,am,K,t​). The allocation space is defined as {am,t​∣am,t,k​∈Ad​,∑k=1Km​​am,t,k​≤1}. 


Mathematical Problem Formulation:

Assume there are a large number M of ads campaigns running concurrently/sequentially. Each ad campaign m contains K≪M ad lines, and we would like to allocate the daily budget limit Qm​ specified by advertisers to Kad lines every day t∈[0,1,⋯,Tm​−1] throughout the ads campaign lasting for Tm​ days. Let the action space for each ad line in the ads campaign m be Ad​=[0,1]. Let am,t,k​ denotes the proportion of budget we assigned to ad line k at time t within ads campaign m, and let am,t​=(am,t,1​,⋯,am,t,K​) be the budget allocation to all K ad lines at day t of the ads campaign m. Thus, the full allocation space is defined as {am,t​∣am,t,k​∈Ad​,∑k=1K​am,t,k​≤1}. Adapting to the combinatorial bandits framework, we consider maintain a set of base arms at ads campaign m as Sm​={(k,a)∣k∈[K],a∈Ad​}. For each base arm (k,a), we denote the expected reward of playing (k,a) as  fm,t,k​(a)=E[Rm,t,k​∣xm,t,k​]+ϵm,t,k​, where ϵm,t,k​ is a mean-zero error term. Then, am,t​ can be rewritten as {(1,am,1,t​),⋯,(Km​,am,Km​,t​)}
 and the expected total reward obtained in round t of ads campaign m can be written as a function of am,t​, such that 
rm,t′​(am,t​)=E∑k=1K​fm,t,k​(am,t,k​),
which is the t

Our problem of interest is to maximize the cumulative reward ∑m=1M​∑t=1T​rm,t′​(am,t​), which can also be written as:
\begin{aligned} \sum_{m=1}^M\sum_{t=1}^T \sum_{k=1}^K f_{m,t,k}(a_{m,t,k})\\ \text{subject to} \sum_{k=1}^{K}a_{m,t,k} \leq Q_m  \forall m, t\end{aligned}
where the cumulative reward is summed over all campaigns/tasks, different ad lines, and across all rounds. 


To address this problem, we plan to extend traditional combinatorial bandits to multi-task settings via a hierarchical model. 
\begin{aligned}\text{Prior: }\quad&\theta\sim \mathbb{P}(\theta)\\ \text{inter-task: }\quad& r_k^{(i)}|x_{k}^{(i)},\theta \sim f(r_k^{(i)}|x_{k}^{(i)},\theta) \\  \text{intra-task: }\quad& R_{t,k}^{(i)} = \sum_{i=1}^K \mathbb{I}(A_{t,k}^{(i)} =a) r_{k,a}^{(i)}+\epsilon_{t,k}^{(i)}\end{aligned}
Within each task, we select action At,k(i)​ via combinatorial bandits by developing a new algorithm from Combinatorial Multi-armed Bandits for Resource Allocation based on Thompson Sampling. [details may need further discussion.]


Questions:

1. Do we plan to model the budget splitting across different ad campaigns? If so, this problem seems to be too complicated. However, even if budget values are pre-specified for each ad campaign, say we allocate Q1​,…,QK​ to the ad campaigns, it is still unrealistic to assume that all tasks share the same action space after discretization. 
2. We may lose some information by discretizing the continuous budget into finite arms. Traditional MAB or CB problem treats different arms as parallel categories, so that each arm are in equal position when doing exploration. However, since there is a natural order between different discretized budget values, regarding all arms as independent categorical values may result in the inefficiency of exploration. Therefore, it might be better to regard the budget as a continuous action, but further investigation is needed to find the most suitable solution.
3. Another concern about Combinatorial Multi-armed Bandits for Resource Allocation is that this paper only handles MAB. We may need to first develop a Contextual version based on TS for combinatorial bandits, and then extend the framework to multi-task settings.
4.  A further concern with combinatorial MAB is that the action space is NK for each task, where N is the number of discretized intervals. There is a trade off between information loss and computation complexity when discretizing the continuous action space.



==> other_derivation.tex <==
\subsection{Posterior Distribution of MTTS-LMM (simple case):}

First, we compute the distribution of $\vY_{1:H}$ given $\vPsi_{1:H}(\vZ_{1:H})$ and $\vthe$, the distribution of $\vY_{1:H}$ given only $\vPsi_{1:H}$, and the distribution of $\vthe$. Note that, $\vPsi_{1:H} = \vZ_{1:H}^{T}\vPhi$. Given $\vthe$, we can write 
\begin{align*}
    \vY_{1:H} = \vZ_{1:H}^{T}\vthe + \epsilon \text{, where } \epsilon \sim \normal(0,\sigma^{2}\vI_{KH}).
\end{align*}
Similarly, given $\vPhi$ and $\vgamma$, we have 
\begin{align*}
    \vthe = \vPhi\vgamma + \nu \text{, where } \nu \sim \normal(0,\sigma_{m}^{2}\vI_{MKN}).
\end{align*}

\noindent Further, given $\vmu_{\vgamma}$, we have
\begin{align*}
    \vgamma = \vmu_{\vgamma} + b   \text{, where } b \sim \normal(0,{\Cov}_{\vgamma}).
\end{align*}
Combining above three equations, we have
\begin{align*}
    \vY_{1:H}|\vPsi_{1:H},\vthe &= \vZ_{1:H}^{T}\vthe + \epsilon,\\
    \vthe &= \vPhi\vmu_{\vgamma} + \vPhi b + \nu,\\
    \vY_{1:H}|\vPsi_{1:H} &= \vPsi_{1:H}\vmu_{\vgamma} + \vPsi_{1:H} b + \vZ_{1:H}^{T} \nu + \epsilon.
\end{align*}
Therefore, we have
\begin{align*}
    \vY_{1:H}|\vPsi_{1:H},\vthe &\sim  \normal(\vZ_{1:H}^{T}\vthe, \sigma^{2}\vI_{KH}),\\
    \vthe &\sim \normal(\vPhi\vmu_{\vgamma},\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_m^2 \vI_{MKN}), \\
    \vY_{1:H}|\vPsi_{1:H} &\sim \normal(\vPsi_{1:H}\vmu_{\vgamma}, \vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}+\sigma^{2}\vI_{KH}).
\end{align*}
Let $\vB \sim \normal(0,\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_m^2 \vI_{MKN})$, we have
\begin{align*}
    \vthe &= \vPhi\vmu_{\vgamma} + \vB,\\
    \vY_{1:H}|\vPsi_{1:H},\vB &\sim \normal(\vPsi_{1:H}\vmu_{\vgamma}+\vZ_{1:H}^{T}\vB,\sigma^{2}\vI_{KH}).
\end{align*}

Then, we compute the posterior distribution of $\vB$ instead of $\vthe$.

\begin{align*}
    \mathds{P}(\vB|\vY_{1:H}) & \propto  \mathds{P}(\vY_{1:H}|\vB)\mathds{P}(\vB)\\
    &\propto  exp\Big(-\frac{1}{2}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}-\vZ_{1:H}^{T}\vB)^{T}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}-\vZ_{1:H}^{T}\vB)\Big)\\
    &\qquad \times exp\Big(-\frac{1}{2}\vB^{T}(\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_m^2\vI)^{-1}\vB\Big)\\
    & \propto  exp\Big(\vB^{T}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}) -\frac{1}{2}\vB^{T}\underbrace{\{(\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_m^2\vI)^{-1}+\frac{1}{\sigma^{2}}\vZ_{1:H}\vZ_{1:H}^{T}\}}_{\tilde{{\Cov}}^{-1}}\vB\Big)\\
    & \sim  \normal(\underbrace{\tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})}_{\vmu(\vB)},\tilde{{\Cov}}).
\end{align*}
Using the Woodbury matrix identity \citep{rasmussen2003gaussian}, we have
\begin{align*}
    \tilde{{\Cov}} & = \bold{G}-\bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}\vZ_{1:H}^T\bold{G},
\end{align*}
where $\bold{G} = \vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_m^2\vI$, 
and 
\begin{align*}
    \vmu(\vB) &= \tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big[\vI_{KH}-\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}\vZ_{1:H}^T\bold{G}\vZ_{1:H}\Big] \frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}\sigma^{2}\vI_{KH}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}).
\end{align*}
Since $\vthe = \vPhi\vmu_{\vgamma} + \vB$, we get the posterior distribution of $\vthe$.
\begin{align*}
    \vthe|\mH \sim \normal(\vPhi\vmu_{\vgamma}+\vmu(\vB),\tilde{{\Cov}}).
\end{align*}
In particular, for each base arm $i \in [MKN]$, the posterior distribution of the base arm-specific parameter $\theta_{i}$ is as follows.
\begin{equation}
    \begin{split}
\theta_{i}|\mH &\sim \mathcal{N}(\hat{\mu}(i),\hat{\sigma}^{2}(i)),\\
\hat{\mu}(i)&=\vx_i^{T}\vmu_{\vgamma}+(\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\vZ_{1:H,i})(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H})^{-1}(\vY_{1:H}-\vPsi_{1:H} \vmu_{\vgamma}),\\
    \hat{\sigma}^{2}(i)&=\vx_i^T{\Cov}_{\vgamma}\vx_i+\sigma_{m}^{2}-(\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\vZ_{1:H,i})(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H})^{-1}(\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\vZ_{1:H,i})^{T}.
    \end{split}
\end{equation}

\noindent For the GP version, we can follow the same derivation, but with the following model assumptions.
\begin{align*}
    \vY_{1:H} &= \vZ_{1:H}^{T}\vthe + \epsilon \text{, where } \epsilon \sim \normal(0,\sigma^{2}\vI_{KH})\\
    \vthe &= \boldsymbol{f}(\Phi) + \nu \text{, where } \nu \sim \normal(0,\sigma_{m}^{2}\vI_{MKN}),\\
    \boldsymbol{f}(\Phi) &\sim \normal(\bar{\vmu}_0,\mathcal{K}) \text{, as } f \sim GP(\mu_0, k(x,x')),
\end{align*} where $\boldsymbol{f}(\Phi)\equiv [f(x_1), \cdots, f(x_{MKN})]^T$, $\bar{\vmu}_0 = [\mu_0(x_1), \cdots, \mu_0(x_{MKN})]^T$, and the $(i,j)$ entry of $\mathcal{K}$ is $k(x_i,x_j)$.


\subsection{Posterior Distribution of MTTS-LMM (cross-effects):} \label{appendix:LLM}

First, we compute the distribution of $\vY_{1:H}$ given $\vPsi_{1:H}(\vZ_{1:H})$ and $\vthe$, the distribution of $\vY_{1:H}$ given only $\vPsi_{1:H}$, and the distribution of $\vthe$. Note that, $\vPsi_{1:H} = \vZ_{1:H}^{T}\vPhi$. Given $\vthe$, we can write 
\begin{align*}
    \vY_{1:H} = \vZ_{1:H}^{T}\vthe + \epsilon \text{, where } \epsilon \sim \normal(0,\sigma^{2}\vI_{KH}).
\end{align*}
Similarly, given $\vPhi$ and $\vgamma$, we have 
\begin{align*}
    \vthe = \vPhi\vgamma + \Lambda^{m}\nu^m + \Lambda^{k}\nu^k,
\end{align*}
where $\Lambda^{m} = diag(\bold{1}_{KN}, \cdots, \bold{1}_{KN})$ is a $MKN \times M$ matrix, $\Lambda^{k} = diag(\bold{1}_{N}, \cdots, \bold{1}_{N})$ is a $MKN \times MK$ matrix, $\nu^m \sim \normal(0,\sigma_{m}^{2}\vI_{M})$, $\nu^k \sim \normal(0,\sigma_{k}^{2}\vI_{MK})$.

\noindent Further, given $\vmu_{\vgamma}$, we have
\begin{align*}
    \vgamma = \vmu_{\vgamma} + b   \text{, where } b \sim \normal(0,{\Cov}_{\vgamma}).
\end{align*}
Combining above three equations, we have
\begin{align*}
    \vY_{1:H}|\vPsi_{1:H},\vthe &= \vZ_{1:H}^{T}\vthe + \epsilon,\\
    \vthe &= \vPhi\vmu_{\vgamma} + \vPhi b + \Lambda_{m}\nu_m + \Lambda_{k}\nu_k,\\
    \vY_{1:H}|\vPsi_{1:H} &= \vPsi_{1:H}\vmu_{\vgamma} + \vPsi_{1:H} b + \vZ_{1:H}^{T} \Lambda_{m}\nu_m + \vZ_{1:H}^{T}\Lambda_{k}\nu_k + \epsilon.
\end{align*}
Therefore, we have
\begin{align*}
    \vY_{1:H}|\vPsi_{1:H},\vthe &\sim  \normal(\vZ_{1:H}^{T}\vthe, \sigma^{2}\vI_{KH}),\\
    \vthe &\sim \normal(\vPhi\vmu_{\vgamma},\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_{m}^{2}\Lambda_{m}\Lambda_{m}^T+\sigma_{k}^{2}\Lambda_{k}\Lambda_{k}^T), \\
    \vY_{1:H}|\vPsi_{1:H} &\sim \normal(\vPsi_{1:H}\vmu_{\vgamma}, \vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H}+\sigma^{2}\vI_{KH}).
\end{align*}
Let $\vB \sim \normal(0,\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_{m}^{2}\Lambda_{m}\Lambda_{m}^T+\sigma_{k}^{2}\Lambda_{k}\Lambda_{k}^T)$, we have
\begin{align*}
    \vthe &= \vPhi\vmu_{\vgamma} + \vB,\\
    \vY_{1:H}|\vPsi_{1:H},\vB &\sim \normal(\vPsi_{1:H}\vmu_{\vgamma}+\vZ_{1:H}^{T}\vB,\sigma^{2}\vI_{KH}).
\end{align*}

Then, we compute the posterior distribution of $\vB$ instead of $\vthe$.

\begin{align*}
    \mathds{P}(\vB|\vY_{1:H}) & \propto  \mathds{P}(\vY_{1:H}|\vB)\mathds{P}(\vB)\\
    &\propto  exp\Big(-\frac{1}{2}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}-\vZ_{1:H}^{T}\vB)^{T}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}-\vZ_{1:H}^{T}\vB)\Big)\\
    &\qquad \times exp\Big(-\frac{1}{2}\vB^{T}(\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_{m}^{2}\Lambda_{m}\Lambda_{m}^T+\sigma_{k}^{2}\Lambda_{k}\Lambda_{k}^T)^{-1}\vB\Big)\\
    & \propto  exp\Big(\vB^{T}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
    &\qquad \qquad -\frac{1}{2}\vB^{T}\underbrace{\{(\vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_{m}^{2}\Lambda_{m}\Lambda_{m}^T+\sigma_{k}^{2}\Lambda_{k}\Lambda_{k}^T)^{-1}+\frac{1}{\sigma^{2}}\vZ_{1:H}\vZ_{1:H}^{T}\}}_{\tilde{{\Cov}}^{-1}}\vB\Big)\\
    & \sim  \normal(\underbrace{\tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})}_{\vmu(\vB)},\tilde{{\Cov}}).
\end{align*}
Using the Woodbury matrix identity \citep{rasmussen2003gaussian}, we have
\begin{align*}
    \tilde{{\Cov}} & = \bold{G}-\bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H}\Big)^{-1}\vZ_{1:H}^T\bold{G},
\end{align*}
where $\bold{G} = \vPhi{\Cov}_{\vgamma}\vPhi^{T}+\sigma_{m}^{2}\Lambda_{m}\Lambda_{m}^T+\sigma_{k}^{2}\Lambda_{k}\Lambda_{k}^T$, 
and 
\begin{align*}
    \vmu(\vB) &= \tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big[\vI_{KH}-\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H}\Big)^{-1}\\
     &\qquad \qquad \qquad \qquad \qquad \qquad \qquad \vZ_{1:H}^T\bold{G}\vZ_{1:H}\Big] \frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H}\Big)^{-1}\sigma^{2}\vI_{KH}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma})\\
     &= \bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H}\Big)^{-1}(\vY_{1:H}-\vPsi_{1:H}\vmu_{\vgamma}).
\end{align*}
Since $\vthe = \vPhi\vmu_{\vgamma} + \vB$, we get the posterior distribution of $\vthe$.
\begin{align*}
    \vthe|\mH \sim \normal(\vPhi\vmu_{\vgamma}+\vmu(\vB),\tilde{{\Cov}}).
\end{align*}
In particular, for each base arm $i \in [MKN]$, the posterior distribution of the base arm-specific parameter $\theta_{i}$ is as follows.
\begin{equation}
    \begin{split}
\theta_{i}|\mH &\sim \mathcal{N}(\hat{\mu}(i),\hat{\sigma}^{2}(i)),\\
\hat{\mu}(i)&=\vx_i^{T}\vmu_{\vgamma}+(\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\Lambda_{m,i}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\Lambda_{k,i}\Lambda_{k}^T\vZ_{1:H})\\
&\qquad \times (\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H})^{-1}(\vY_{1:H}-\vPsi_{1:H} \vmu_{\vgamma}),\\
    \hat{\sigma}^{2}(i)&=\vx_i^T{\Cov}_{\vgamma}\vx_i+\sigma_{m}^{2} + \sigma_{k}^{2}-(\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\Lambda_{m,i}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\Lambda_{k,i}\Lambda_{k}^T\vZ_{1:H})\\
    &\qquad \times (\sigma^{2}\vI_{KH}+\vPsi_{1:H}{\Cov}_{\vgamma}\vPsi^{T}_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\Lambda_{m}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\vZ_{1:H}^{T}\Lambda_{k}\Lambda_{k}^T\vZ_{1:H})^{-1}\\
    &\qquad \times (\vx_i{\Cov}_{\vgamma}\vPsi_{1:H}^{T} + \sigma_{m}^{2}\Lambda_{m,i}\Lambda_{m}^T\vZ_{1:H}+\sigma_{k}^{2}\Lambda_{k,i}\Lambda_{k}^T\vZ_{1:H})^{T}.
    \end{split}
\end{equation}


\subsection{One-Step Posterior Derivation of Gaussian Process} 
Now we focus on deriving the posterior distribution for parameter updates in Equation \eqref{eq:8}.
\begin{equation}
    \begin{alignedat}{2}
        &\text{(Prior)} \quad
        \quad\quad\quad \quad\quad \quad\quad  f&&\sim G P\left(0, k\left(x, x^{\prime}\right)\right), \\
        &\text{(Generalization)} \quad
        \; \vthe \mid \{x_{m, k, a}\}, f&&=f\left(x_{m, k, a}\right)+\vdelta  \\
        &\text{(Observation)} \quad
        \;\quad\quad \;   Y_{m, k, a, t} && =\theta_{m, k, a}+\epsilon_{m, k, a, t}, \forall (k,a)\in A_{m,t},\\
        &\text{(Reward)} \quad \quad\quad
        \quad\quad \quad \; R_{m,t} &&= \sum_{(k,a)\in A_{m,t}}Y_{m,k,a,t},
    \end{alignedat}
\end{equation}


Similar to Appendix \ref{appendix:LLM}, we have 
\begin{equation*}
\begin{aligned}
    \vY_{1:H} &= \vZ_{1:H}^{T}\vthe + \epsilon \text{, where } \epsilon \sim \normal(0,\sigma^{2}\vI_{KH})\\
    \vthe & = f(\vPhi) + \nu \text{, where } \nu \sim \normal(0,\sigma_{m}^{2}\vI_{MKN})\\
    f(\vPhi)& \sim \mathcal{N}(\vmu_f,\boldsymbol{\mathcal{K}}_f)
\end{aligned}
\end{equation*}
where $\boldsymbol{\mathcal{K}}_f$ is a $MKN$ by $MKN$ matrix with $\boldsymbol{\mathcal{K}}_{ij} = k(\boldsymbol{x}_i,\boldsymbol{x}_j)$, and $k(\cdot,\cdot)$ is a pre-specified kernel function.

For simplicity of notations, we define $\vthe = \vmu_f +\vB$, where $\vB\sim \mathcal{N}(0,\boldsymbol{\mathcal{K}}_f+\sigma_{m}^{2}\vI_{MKN})$. Therefore, we have
\begin{align*}
    \vthe &= \vmu_f + \vB,\\
    \vY_{1:H}|\vPsi_{1:H},\vB &\sim \normal(\vZ_{1:H}^{T}\vmu_f+\vZ_{1:H}^{T}\vB,\sigma^{2}\vI_{KH}).
\end{align*}

Then, the posterior distribution of $\vB$ can be similarly derived as

\begin{align*}
    \mathds{P}(\vB|\vY_{1:H}) & \propto  \mathds{P}(\vY_{1:H}|\vB)\mathds{P}(\vB)\\
    & \propto  exp\Big(\vB^{T}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vZ_{1:H}^T\vmu_{f})\\
    &\qquad \qquad -\frac{1}{2}\vB^{T}\underbrace{\{(\boldsymbol{\mathcal{K}}_f+\sigma_{m}^{2}\vI_{MKN})^{-1}+\frac{1}{\sigma^{2}}\vZ_{1:H}\vZ_{1:H}^{T}\}}_{\tilde{{\Cov}}^{-1}}\vB\Big)\\
    & \sim  \normal(\underbrace{\tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vZ_{1:H}^T\vmu_{f})}_{\vmu(\vB)},\tilde{{\Cov}}).
\end{align*}
Using the Woodbury matrix identity \citep{rasmussen2003gaussian}, we have
\begin{align*}
    \tilde{{\Cov}} & = \bold{G}-\bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vZ^T_{1:H}\boldsymbol{\mathcal{K}}_f\vZ_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}\vZ_{1:H}^T\bold{G},
\end{align*}
where $\bold{G} = \boldsymbol{\mathcal{K}}_f+\sigma_{m}^{2}\vI_{MKN}$, 
and 
\begin{align*}
    \vmu(\vB) &= \tilde{{\Cov}}\vZ_{1:H}\frac{1}{\sigma^{2}}(\vY_{1:H}-\vZ_{1:H}\vmu_{f})\\
     &= \bold{G}\vZ_{1:H}\Big(\sigma^{2}\vI_{KH}+\vZ^{T}_{1:H}\boldsymbol{\mathcal{K}}_f\vZ_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H}\Big)^{-1}(\vY_{1:H}-\vZ_{1:H}\vmu_{f}).
\end{align*}

Since $\vthe = f(\vPhi) + \vB$, we can finally obtain the posterior distribution of $\vthe$ as
\begin{align*}
    \vthe|\mH \sim \normal(\vmu_f+\vmu(\vB),\tilde{{\Cov}}).
\end{align*}

In particular, for each base arm $i \in [MKN]$, the posterior distribution of the base arm-specific parameter $\theta_{i}$ is as follows.
\begin{equation}
    \begin{split}
\theta_{i}|\mH &\sim \mathcal{N}(\hat{\mu}(i),\hat{\sigma}^{2}(i)),\\
\hat{\mu}(i)&=\mu(x_i)+(k(x_i,\vPsi_{1:H}) + \sigma_{m}^{2}\vZ_{1:H,i})(\sigma^{2}\vI_{KH}+\vZ^T_{1:H}\boldsymbol{\mathcal{K}}_f\vZ_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H})^{-1}(\vY_{1:H}-\vZ_{1:H}\vmu_{f}),\\
    \hat{\sigma}^{2}(i)&=k(x_i,x_i)+\sigma_{m}^{2}-(k(x_i,\vPsi_{1:H}) + \sigma_{m}^{2}\vZ_{1:H,i})(\sigma^{2}\vI_{KH}+\vZ^T_{1:H}\boldsymbol{\mathcal{K}}_f\vZ_{1:H}+\sigma_{m}^{2}\vZ_{1:H}^{T}\vZ_{1:H})^{-1}(k(x_i,\vPsi_{1:H}) + \sigma_{m}^{2}\vZ_{1:H,i})^{T}.
    \end{split}
\end{equation}



\begin{comment}
This the above Bayesian hierarchical model is equivalent to 
\begin{equation}
    \begin{alignedat}{2}
        &\text{(Prior)} \quad
        \quad\quad\quad \quad\quad \quad\quad  f&&\sim G P\left(0, k\left(x, x^{\prime}\right)\right), \\
        &\text{(Observation)} \quad
        \;\quad\quad \;   Y_{m, k, a, t} && =f(x_{m, k, a}) + \delta_m + \delta_k +\epsilon_{m, k, a, t}, \forall (k,a)\in A_{m,t},
    \end{alignedat}    
\end{equation}
where $\delta_m\sim \mathcal{N}\left(0, \sigma_m^2\right)$, $\delta_k\sim \mathcal{N}\left(0, \sigma_k^2\right)$, and $\epsilon_{m,k,a,t}\sim \mathcal{N}\left(0, \sigma^2\right)$.

Another expression:
\begin{equation}
    \begin{alignedat}{2}
        &\text{(Prior)} \quad
        \quad\quad\quad \quad\quad \quad\quad  f&&\sim G P\left(0, k\left(x, x^{\prime}\right)\right), \\
        &\text{(Generalization)} \quad
        \; \gamma_{m, k, a} \mid x_{m, k, a}, f&&=f\left(x_{m, k, a}\right)+\delta_m, \forall m,k,a,  \\
        &\text{(Generalization)} \quad
        \; \theta_{m, k, a} \mid \gamma_{m, k, a}&&=\gamma_{m, k, a}+\delta_k, \forall m,k,a,  \\
        &\text{(Observation)} \quad
        \;\quad\quad \;   Y_{m, k, a, t} && =\theta_{m, k, a}+\epsilon_{m, k, a, t}, \forall (k,a)\in A_{m,t},\\
        &\text{(Reward)} \quad \quad\quad
        \quad\quad \quad \; R_{m,t} &&= \sum_{(k,a)\in A_{m,t}}Y_{m,k,a,t},
    \end{alignedat}
\end{equation}
\end{comment}



\begin{comment}
We first start from a simpler version where $\delta_k = 0$, i.e. there is no ad line level random effect. 

Define all of the historical data up to round $t$ as $\mathcal{H}_t:= \mathcal{H}_{t-1}\cup \{X_{m,k,a}, A_{m,k,a,t}, Y_{m,k,a,t}\}$, where $A_{m,k,a,t}$ saves the $(k,a)$ tuple that denotes the budget proportion chosen for ad line $k$.


Define $\boldsymbol{Y}_{1:H} = (\boldsymbol{Y}_1^T, \dots, \boldsymbol{Y}_t^T)^T \in \mathbb{R}^{MKAt}$ as a vector containing all of the observed rewards from the first $t$ rounds. Define $\boldsymbol{\phi}_t = \{x_{m,k,a}\}$ as the features of all $(m,k,a)$ tuples collected from round $t$, and further define $\boldsymbol{\Phi}_{1:H} = (\boldsymbol{\phi}_1^T,\dots, \boldsymbol{\phi}_t^T)^T$ as the collection of all contextual information up to round $t$. Note that $\boldsymbol{\Phi}_{1:H}$ is different from $\boldsymbol{\phi} = \{x_{m,k,a}\}_{\forall m,k,a}$, where the latter denotes the collection of features for all $(m,k,a)$, regardless of the repeated info across different rounds. Lastly, we define $\boldsymbol{Z}_{1:H}\in \mathbb{R}^{MKA\times MKAt}$, such that the $(j,a)$th entry of $\boldsymbol{Z}_{1:H}$ is $\boldsymbol{1}\{i(a) =j\}$, where $i(a)$ is the item index of the $a$th observed reward in $\boldsymbol{Y}_{1:H}$.





\begin{equation}
    \begin{alignedat}{2}
        &\boldsymbol{Y}_{1:H} = \boldsymbol{Z}_{1:H}\boldsymbol{\theta} + \boldsymbol{\epsilon}_{1:H},  \quad &&\boldsymbol{\epsilon}_{1:H}\sim \mathcal{N}\left(0, \sigma^2 \boldsymbol{I}\right), \\
        &\boldsymbol{\theta} = f(\boldsymbol{\Phi}) + \boldsymbol{\delta_m}, \quad &&\boldsymbol{\delta_m} \sim \mathcal{N}\left(0, \Sigma_m\right)  \\
        &f(\boldsymbol{\Phi}) \sim \mathcal{N}\left(\boldsymbol{\mu},  \boldsymbol{\mathcal{K}}\right) && 
    \end{alignedat}
\end{equation}

Therefore, 

\subsubsection{$\pi(\boldsymbol{\theta}|\mathcal{H})$}
\begin{equation}
\begin{aligned}
    \pi(\theta_{m,k,a}|\mathcal{H}) 
    &\propto \prod_{m,k,a,t}p(y_{m,k,a,t}|\theta_{m,k,a},\sigma^2)\cdot \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma^2_k)\cdot \prod_{m,k,a}p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma^2_m)\cdot \prod_{m,k,a}p(f|x_{m,k,a})\\
    &    \\ 
    &    \\ 
    &    \\ 
    &    \\ 
\end{aligned}
\end{equation}


\end{comment}
\begin{comment}
\subsubsection{$\pi(\boldsymbol{f}|\mathcal{H})$}
First, we derive the posterior distribution of the Gaussian process $\boldsymbol{f} = \{f_{m,k,a}\}$. Since $f|x_{m,k,a}\sim\mathcal{N}(0,\mathcal{K}_{m,k,a})$, we have
\begin{equation}
\begin{aligned}
    \pi(f|\mathcal{H}) &\propto \prod_{m,k,a,t}p(y_{m,k,a,t}|\theta_{m,k,a},\sigma^2)\cdot \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma_k^2)\cdot \prod_{m,k,a}p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma_m^2)\cdot \prod_{m,k,a}p(f|x_{m,k,a})\\
    &\propto \prod_{m,k,a} p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma_m^2)\cdot \prod_{m,k,a}p(f|x_{m,k,a})\\
    & \propto \exp\Big\{-\sum_{m,k,a}\frac{1}{2\sigma_m^2}\big(\gamma_{m,k,a}-f\big)^2\Big\}\cdot \exp\Big\{-\sum_{m,k,a}\frac{1}{2\mathcal{K}_{m,k,a}}f^2\Big\}
\end{aligned}
\end{equation}
After some manipulations, we can derive
$$
\pi(\boldsymbol{f}|\mathcal{H}) \sim \mathcal{N}\Big(\sigma_m^{-2} \big(\mathcal{K}^{-1} + \sigma_m^{-2}I\big)^{-1}\boldsymbol{\gamma}, \big(\mathcal{K}^{-1} + \sigma_m^{-2}I\big)^{-1}\Big).
$$

\subsubsection{$\pi(\boldsymbol{\gamma}|\mathcal{H})$}

\begin{equation}
\begin{aligned}
    \pi(\gamma_{m,k,a}|\mathcal{H}) &\propto \prod_{m,k,a,t}p(y_{m,k,a,t}|\theta_{m,k,a},\sigma^2)\cdot \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma^2_k)\cdot \prod_{m,k,a}p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma^2_m)\cdot \prod_{m,k,a}p(f|x_{m,k,a})\\
    &\propto \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma^2_k)\cdot \prod_{m,k,a}p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma^2_m)\\
    & \propto \exp\Big\{-\sum_{m,k,a}\frac{1}{2\sigma_k^2}\big(\theta_{m,k,a}-\gamma_{m,k,a}\big)^2\Big\} \cdot \exp\Big\{-\sum_{m,k,a}\frac{1}{2\sigma_m^2}\big(\gamma_{m,k,a}-f\big)^2\Big\}\\
    & \propto \exp\Big\{\frac{1}{\sigma_m^2}\gamma_{m,k,a}^2 + \frac{1}{\sigma_k^2}\gamma_{m,k,a}^2 - \frac{2}{\sigma_k^2}\theta_{m,k,a}\cdot \gamma_{m,k,a}- \frac{2}{\sigma_m^2}f\cdot\gamma_{m,k,a} \Big\}
\end{aligned}
\end{equation}
After some manipulations, we have
$$
\pi(\boldsymbol{\gamma}|\mathcal{H}) \sim \mathcal{N}\Big(\big(\sigma_m^{-2} +\sigma_k^{-2}\big)^{-1} \big(\sigma_k^{-2}\boldsymbol{\theta}+\sigma_m^{-2}\boldsymbol{f}\big), \big(\sigma_m^{-2} + \sigma_k^{-2}\big)^{-1} I\Big).
$$

\subsubsection{$\pi(\boldsymbol{\theta}|\mathcal{H})$}

\begin{equation}
\begin{aligned}
    \pi(\theta_{m,k,a}|\mathcal{H}) 
    &\propto \prod_{m,k,a,t}p(y_{m,k,a,t}|\theta_{m,k,a},\sigma^2)\cdot \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma^2_k)\cdot \prod_{m,k,a}p(\gamma_{m,k,a}|x_{m,k,a},f,\sigma^2_m)\cdot \prod_{m,k,a}p(f|x_{m,k,a})\\
    &\propto \prod_{m,k,a,t}p(y_{m,k,a,t}|\theta_{m,k,a},\sigma^2)\cdot \prod_{m,k,a}p(\theta_{m,k,a}|\gamma_{m,k,a},\sigma^2_k)\\
    & \propto \exp\Big\{-\sum_{m,k,a,t}\frac{1}{2\sigma^2}\big(y_{m,k,a,t}-\theta_{m,k,a}\big)^2\Big\}\cdot \exp\Big\{-\sum_{m,k,a}\frac{1}{2\sigma_k^2}\big(\theta_{m,k,a}-\gamma_{m,k,a}\big)^2\Big\} \\
    & \propto \exp\Big\{-\sum_{t}\frac{1}{2\sigma^2}\big(y_{m,k,a,t}-\theta_{m,k,a}\big)^2\Big\}\cdot \exp\Big\{-\frac{1}{2\sigma_k^2}\big(\theta_{m,k,a}-\gamma_{m,k,a}\big)^2\Big\} \\
    & \propto \exp\Big\{\frac{t}{\sigma^2}\theta_{m,k,a}^2 + \frac{1}{\sigma_k^2}\theta_{m,k,a}^2 - \frac{2}{\sigma^2}\sum_t y_{m,k,a,t}\cdot \theta_{m,k,a}- \frac{2}{\sigma_k^2}\gamma_{m,k,a}\cdot\theta_{m,k,a} \Big\}
\end{aligned}
\end{equation}
After some manipulations, we have
$$
\pi(\boldsymbol{\theta}|\mathcal{H}) \sim \mathcal{N}\Big(\big(t\sigma^{-2} +\sigma_k^{-2}\big)^{-1} \big(\sigma^{-2}\boldsymbol{Y}_t+\sigma_k^{-2}\boldsymbol{\gamma}\big), \big(t\sigma^{-2} + \sigma_k^{-2}\big)^{-1} I\Big),
$$
where $\boldsymbol{Y}_t$ is a $MK(N+1)$ by $MK(N+1)$ diagonal matrix with the $(m,k,a)$th diagonal elements taking $\sum_{t'=1}^t y_{m,k,a,t}$.
\end{comment}


\begin{comment}
\subsubsection{$\pi(R_{m,t}|\mathcal{H})$}

Since $Y_{m,k,a,t}= \theta_{m,k,a}+ \epsilon_{m,k,a,t}$, the posterior of $Y_{m,k,a,t}$ is thus
\begin{equation}
    \pi(Y_{m,k,a,t}|\mathcal{H}) \sim \mathcal{N}\Big(\big(t\sigma^{-2} +\sigma_k^{-2}\big)^{-1} \big(\sigma^{-2}\sum_{t'=1}^t y_{m,k,a,t}+\sigma_k^{-2}\gamma_{m,k,a}\big), \big(t\sigma^{-2} + \sigma_k^{-2}\big)^{-1}+ \sigma^2\Big)
\end{equation}
Thus, the posterior distribution of $R_{m,t}$ can be derived accordingly as follows
\begin{equation}
    \pi(R_{m,t}|\mathcal{H}) \sim \mathcal{N}\Big(\sum_{k,a}\big(t\sigma^{-2} +\sigma_k^{-2}\big)^{-1} \big(\sigma^{-2}\sum_{t'=1}^t y_{m,k,a,t}+\sigma_k^{-2}\gamma_{m,k,a}\big), \sum_{k}(N+1)\big(t\sigma^{-2} + \sigma_k^{-2}\big)^{-1}+ K(N+1)\sigma^2\Big)
\end{equation}

\end{comment}



